CLAIR: A Contract-based Framework for Developing Resilient CPS Architectures

Industrial cyber-infrastructure is normally a multilayered architecture. The purpose of the layered architecture is to hide complexity and allow independent evolution of the layers. In this paper, we argue that this traditional strict layering results in poor transparency across layers affecting the ability to significantly improve resiliency. We propose a contract-based methodology where components across and within the layers of the cyber-infrastructure are associated with contracts and a light-weight resilience manager. This allows the system to detect faults (contract violation monitored using observers) and react (change contracts dynamically) effectively. It results in (1) improving transparency across layers; helps resiliency, (2) decoupling fault-handling code from application code; helps code maintenance, (3) systematically generate error-free fault handling code; reduces development time. Using an industrial case study, we demonstrate the proposed methodology.

==> content/bio.tex <==
\begin{IEEEbiography}{Sidharta Andalam}
		Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Daniel  Jun Xian Ng }
	Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Arvind Easwaran}
	Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Karthikeyan Thangamariappan}
	Biography text here.
\end{IEEEbiography}

==> content/sec_discussion.tex <==

\begin{itemize}
	\item We did not elaborate on the fault channel used for communication between resilience managers.
	\item We assumed platform technologies such as clock synchronisation,....
	\item RaspberryPi 3.3 volts to 24 volts Red Factory. Bridging hardware is ...
	\item 
	
\end{itemize}

==> content/sec_quanRes.tex <==

We start with the assumption that faults are inevitable. In general, it is not practical to develop a foolproof resilient system. Rather, we  prepare for response to faults  the application demands and the availability of the cyber-infrastructure resources. 
 Figure~\ref{fig:PerVStime} depicts  the performance of a system (or a component) over time in the presence of a fault.
 A fault has occurred at time~$t_0$. It was detected at $t_1$
 which initiated a recovery process. Furthermore, we 
 define \emph{recovery period} as the time from fault detection to the time when the functionality was recovered to the maximum extent. This can be
  either fully or partially recovered state as shown in the figure. 


\begin{figure}[bthp]
	\centering
	\includegraphics[width=0.98\columnwidth]{./figures/PerformVSTime.jpg}
	\caption{\label{fig:PerVStime} Performance degrades due to a fault. however, based on the fault and the recovery strategy it is possible to fully recover from a fault. 
	}
\end{figure}

Due to the heterogeneous nature of the CPS infrastructure (see Figure~\ref{fig:CILayers}) a multi-dimensional metric is required to quantitatively assess the  resiliency of the system. 
The challenge is to develop a sensible abstraction across layers,
while respecting the richness of the cyber-infrastructure.

\subsection{The need for a new resilience metric}

\textbf{Runtime optimization:} Optimizing software applications based on the underlying fault-prone architecture is unaddressed, due to the lack of abstractions that capture the complex interactions between components within and across layers of a cyber-infrastructure. E.g., gcc does not consider the reliability of the registers.

\textbf{Understanding sensitivity:} Relate component-level properties to system-level properties. This helps us to understand the sensitivity of the system-level properties to the changes at component-level. 
E.g., impact of an intermittent fault of an infrared sensor on the color-detection application

\textbf{Design-time optimization:} Explore cost-effective solutions to improve reliability for a given application. This can be done at design time to identify bottlenecks and take corrective actions early. E.g. alternative sensors such as weight for infrared/color sensor.


\subsection{Proposed resilience metric}

We discuss the abstractions that enable us to reason about the performance and resiliency of a system. The abstract metric involves (1) Availability, (2) Demand, (3) Utilisation, (4) Performance, and (5) Resilience.\\

\noindent{\textbf{Availability.}} Describes the availability of the component based on the actions such as faults and internal repairs/maintenance.
A profile of a permanent fault is shown in Figure~\ref{fig:ProfAvailVStime}.
The availability profile is formally described  using Equation~\ref{equ:avail}.
Similarly, we can formally define the availability of a component during an intermittent fault and  different/recovery profiles that are shown in Figure~\ref{fig:ProfAvailVStime}.

\begin{figure}[bthp]
	\centering
	\includegraphics[width=0.98\columnwidth]{./figures/AvailVSTime.jpg}
	\caption{\label{fig:ProfAvailVStime} Availability of a component in the presence of a fault or/and repairs.
	}
\end{figure}

\begin{equation}
\tcbhighmath[boxsep=0mm, width=1cm]{
	\small
	\avalSym(t)=\left\{
	\begin{array}{@{}lll@{}}
	1, & \text{when}~t \le t_1 \\
	0, & otherwise \\
	\end{array}
	\right.
}
\label{equ:avail}
\end{equation}

\noindent{\textbf{Demand.}} The need to use the component. Generally this is a form of requirement from the layers above.
It can be described as a continuous function, denoted as $\dmndSym(t)$.
Examples of a periodic and aperiodic demand profiles are shown in Figure~\ref{fig:ProfDemandVStime}.

\begin{figure}[bthp]
	\centering
	\includegraphics[width=0.98\columnwidth]{./figures/DemandVSTime.jpg}
	\caption{\label{fig:ProfDemandVStime} Example demand profiles on a component.
	}
\end{figure}


\noindent{\textbf{Performance}} is the measure of meeting the demands, denoted as $\perfSym(t)$.
Performance is high (1), if all the demands are met. 
E.g., in Fig.~\ref{fig:PerUtiVSTime} the demand is high between $t_1$ and $t_2$. During this period, the component is always available.
In contrast, after $t_2$ there is no demand. 
Based on Eq.~\ref{equ:Perf}, the performance is high as all demands were met. 



\begin{equation}
\tcbhighmath[boxsep=0mm, width=1cm]{
	\small
	\perfSym(t)=\left\{
	\begin{array}{@{}lll@{}}
	1, & \text{when}~\avalSym(t) - \dmndSym(t) \ge 0 \\
	\avalSym(t) / \dmndSym(t), & otherwise \\
	\end{array}
	\right.
}
\label{equ:Perf}
\end{equation}

\noindent{\textbf{Utilisation}} is the measure of resource usage (1=best, 0=worst). It will be used during optimisation to improve performance.  It  is illustrated using Fig.~\ref{fig:PerUtiVSTime} and formally described using Eq.~\ref{equ:Util}. 

\begin{equation}
\tcbhighmath[boxsep=0mm, width=1cm]{
	\small
	\utilSym(t)=\left\{
	\begin{array}{@{}lll@{}}
	1, & \text{when}~\avalSym(t) \le \dmndSym(t) \\
	\dmndSym(t) / \avalSym(t), & otherwise \\
	\end{array}
	\right.
}
\label{equ:Util}
\end{equation}


\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.98\columnwidth]{./figures/PerUtiVSTime.jpg}
	\caption{\label{fig:PerUtiVSTime} Given availability and demand, 
		we can compute performance and utilization.	}
\end{figure}


\noindent{\textbf{Resilience.}} Given the performance of a component/system without any faults ($\perfSym_{norm}$) and with faults ($\perfSym_{fault}$),
the resilience over a period $T$ can be quantified as area under the curve $\perfSym_{fault}$ w.r.t. $\perfSym_{norm}$.
It is described by Eq.~\ref{equ:resil} and illustrated using Eq.~\ref{fig:ResilVStime}.

\begin{equation}
\tcbhighmath[boxsep=0mm, width=1cm]{
\resiSym^{[t_x,t_y]} = \int_{t_x}^{t_y} \perfSym_{fault}(t) / \perfSym_{norm}(t)
}
\label{equ:resil}
\end{equation}


\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.98\columnwidth]{./figures/ResilVStime.jpg}
	\caption{\label{fig:ResilVStime} The resiliency of the system over the period $[t_x, t_y]$ under fault $f_1(t)$ is $0.\dot{6}  = (2/3) / 1 $.	(Scale: Perfect resiliency (1) and no resiliency (0)).
	}
\end{figure}


\subsection{Applying the metric across layers}

In the previous section, we discussed about the availability and the demand of a component. 
For the 3-layered cyber infrastructure (see Fig.~\ref{fig:CILayers}), our intuition is that the requirements of a layer can be translated into demand(s)
on the availability of the resources at a lower layer, see Table~\ref{tab:xLayerMetric}.
For example, end-to-end timing requirements from the application can be translated to scheduler deadlines of the platform layer. 

\begin{table}[bhtp]
	\input{./tables/xlayerAnD.tex}
	\caption{\label{tab:xLayerMetric} Availability of resources and demand on resources across layers}
\end{table}



==> content/sec_reconfiguration.tex <==
	Dynamic reconfiguration consists of modifying the system during runtime. 
	However, guided by the contracts, we abstract the changes in the 
	cyber-infrastructure as  two types of  reconfigurations.
	
	
	\textbf{1. Application-level reconfiguration:}
	The state of the application is described by an ordered set of contracts currently
	selected by the components to execute their behaviour. 
	For the running example, the ordered set of components
	is $[C_1, C_2, \dots, C_7]$.
	 The initial state of the application can be dictated by the contracts active in each component as $[\conSym_{C_1}^{ 1},\conSym_{C_2}^{1},  \dots \conSym_{C_7}^{2}] $.
	 % Note that each component has only one active contract at any give time.   
	  Any \emph{application-level reconfiguration} is a transition from one application state to another.
	This state transition occurs when a fault is detected (violation of a contract) and a new contract is adopted by a component.
	
	\textbf{2. Platform-level reconfiguration:} As described earlier, the platform layer consists of computational and communicational platforms. Once again, the state of the platform can be described as an ordered set of contracts. 
	Any \emph{platform-level reconfiguration} is a transition from one platform state to another. E.g., due to high network traffic the contract $\conSym_{N_3}^{}$ needed to be re-negotiated  to $\conSym_{N_3}^{\prime}$, representing a reconfiguration at platform level. Note, this may or may not lead to an application level reconfiguration.

==> content/sec_translate2Ccode.tex <==
In the previous section, we used high-level models such as \ac{FSM}, \ac{TA} and \ac{HA} to express observers. In this section, we discuss  existing model-based automatic code generation techniques for automatically generating  low-level synthesisable code from the high-level models.

Plethora of work exists on synthesis of \acp{FSM} to software description languages such as C, C++, Java, etc., and hardware description languages such as VHDL~\cite{Kam1996,SMCtool}. We focus on synthesising higher level models such as \ac{TA} and \ac{HA}.



\subsection{\acf{TA} -  modelling and synthesis}
Timed automaton extends a \ac{FSM} with real-valued clock to capture the physical time. The transitions between states are guarded by conditions that compare the value of the clocks against integers~\cite{Alur:1994}. 
The timed automata model was extended by data variables, executable tasks and by allowing parallel composition of \acp{TA} to form a network~\cite{Amnell2002}. This made it possible to model practical applications. UPPAAL is a well-known tool for modelling, simulation and validation of systems that are modelled as a  network of timed automata~\cite{UppaalTool}.


In general, behaviour of a \ac{TA} is \emph{non-deterministic.} Several transitions may be enabled in a state, which introduces non-determinism. 
This property is not desired for code-generation as most of our computation platforms are deterministic.
As a simple solution, the transitions are assigned with static priorities 
so that the highest enabled transition is always chosen. This is enforced by using deterministic operational semantics~\cite{Amnell2002}. 

The restriction that the value of clocks can be compared against integers only (i.e., not real values) leads to the applicability of discrete-time model, which can be translated to ordinary finite automata~\cite{Alur:1994}. 
In contrast, \ac{HA} does not impose any such conditions. Thus, the translation from continuous-time to discrete-time semantics introduces new challenges.

\subsection{\ac{HA} -  modelling and synthesis}

\acf{HA} is more expressive than \ac{TA} because the continuous variables are described by a set of differential equations. Furthermore, there are no restrictions on the conditions that are enabling the transitions between states. 
Commercial tools such as Simulink's Stateflow~\cite{SimulinkTool} and academic tools such at Ptolemy~\cite{Eker2003,PtolemyTool} can be used for modelling and simulation of hybrid systems. 

The non-determinism which occurs when several transitions may be enabled in a state can be handled using fixed priorities~\cite{Kim2003,Malik2015}.
Importantly, most existing tools rely on numeric solvers that are invoked during runtime for solving the differential equations. This is not ideal for guaranteeing real-time response which is a requirement for model-in-the-loop based validation~\cite{Malik2015}. With a few more semantic restrictions, an \ac{HA} can be translated to a finite automaton from which models such as IEC~61499~\cite{Malik2017} and C-code~\cite{Kim2003,Malik2015}  can  be generated automatically. 
In this paper, we manually translate observers to IEC~61499 standard and then use a synchronous compiler to generate executable C code~\cite{Yoong2015}.
% We hope to automate this process in near future.


%EXAMPLE HA TO FSM TO C-CODE

==> results/faultDetection.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.15,
    legend style={at={(0.5,1.1)},
      anchor=north,legend columns=-1},
    ylabel={Average fault detection time (ms)},
    symbolic x coords={BM1,BM2,BM3,BM4,BM5, BM6},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {(BM1,7) (BM2,9) (BM3,5) (BM4,6) (BM5,5) (BM6,8)};
\addplot coordinates {(BM1,5) (BM2,8) (BM3,4) (BM4,7) (BM5,5) (BM6,6)};
\legend{Traditional, Proposed (CLAIR)}
\end{axis}
\end{tikzpicture}

==> results/faultRecovery.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.15,
    legend style={at={(0.5,1.1)},
      anchor=north,legend columns=-1},
    ylabel={Average fault recovery time (ms)},
    symbolic x coords={BM1,BM2,BM3,BM4,BM5, BM6},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {(BM1,7) (BM2,9) (BM3,5) (BM4,6) (BM5,5) (BM6,8)};
\addplot coordinates {(BM1,5) (BM2,8) (BM3,4) (BM4,7) (BM5,5) (BM6,6)};
\legend{Traditional, Proposed (CLAIR)}
\end{axis}
\end{tikzpicture}

==> results/memorySize.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar, scale, width=0.9\columnwidth, height=5cm, 
    enlargelimits=0.15,
    legend style={at={(0.5,1.17)},
      anchor=north,legend columns=-1},
    ylabel={Memeory consumption (MB)},
    symbolic x coords={RP1,RP2,RP3,RP4,BB1, BB2},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {(RP1,7) (RP2,9) (RP3,5) (RP4,6) (BB1,5) (BB2,8)};
\addplot coordinates {(RP1,5) (RP2,8) (RP3,4) (RP4,7) (BB1,5) (BB2,6)};
\legend{Traditional, Proposed (CLAIR)}
\end{axis}
\end{tikzpicture}

==> results/normalExecution.tex <==

\begin{tikzpicture}[domain=0:100,xscale=1,yscale=1]



\draw[step=0.5cm,color=gray] (0,0) grid (11,5);
%\draw[step=1cm, color=black!60, thick] (0,0) grid (3,1.5);
\draw[->,  ultra thick] (-0.2,0) -- (12.0,0) node[right, text width=1.5cm] {Relative time (in~ms)};


\foreach \x/\xtext in {0/0, 1/400, , 2/800, 3/1200, 4/1600, , 5/2000, 6/2400, 7/2800, 8/3200, 9/3600, 10/4000 , 11/4400  }
\draw[shift={(\x,0)}] (0pt,2pt) -- (0pt,-2pt) node[below] {$\xtext$};

\foreach \y/\ytext in {4.5/comp.,4/$rr$ }
\draw[shift={(0,\y)}]  node[left] {$\ytext$};

%\draw[-&amp;gt;] node[left] {\scriptsize $0$} (0,0) -- (2.5,0)
%    node[below right] {$u$};
%\draw[&amp;lt;-&amp;gt;] (0,-1) -- (0,1.5)
%    node[left] {$x_k$};

%data

\draw[line width=0.7mm, ultra thick] (0.5,0.5) -- (1.2,0.5); %-1
%\draw[line width=0.5mm] (0.25,0) -- (1,0); %0
%\draw[line width=0.5mm] (1,1) -- (2.5,1); %2
%\draw[fill=white] (0,-0.5) circle (0.25mm);
%\draw[fill=black] (0.25,-0.5) circle (0.25mm);
%\draw[fill=white] (0.25,0) circle (0.25mm);
%\draw[fill=black] (1,0) circle (0.25mm);
%\draw[fill=white] (1,1) circle (0.25mm);
%\draw[fill=black] (2.5,1) circle (0.25mm);



\end{tikzpicture}





==> tables/tab_compareArch.tex <==
\begin{table*}[thbp]
	\centering
	\caption{\label{tab:exResArchs}Qualitative analysis of existing architectures}
	\scriptsize
	\begin{tabular}{ m{1.7cm}|m{2.2cm}|m{2.3cm}|m{2.3cm}|m{1.7cm}|m{1.5cm}}\hline
		\textbf{Architecture}
		& \textbf{Example application}
		& \textbf{Fault-detection techniques}
		& \textbf{Fault-detection expressiveness}
		& \textbf{Cross-layer interaction}
		& \textbf{Code intertwined}
		\\\hline
		RIAPS~\cite{Eisele2017} 
		& Discovery service 
		& Heartbeats, timestamps
		& Low
		& None
		& Yes
		\\\hline
		iLand~\cite{Valls2013} 
		& Video surveillance 
		& Not the focus
		& Not the focus
		& None
		& Unknown
		\\\hline
		For IEC~61499~\cite{Vyatkin2017}
		& Baggage handling system
		& Monitor events and data and using ontology
		& Low
		& None
		& No
		\\\hline
		For IEC~61499~\cite{Steinegger2013}
		& Injection moulding machine  
		& Monitor events and data
		& Low
		& None
		& No
		\\\hline
		CLAIR (this~paper)
		& Factory assembly line sorter  
		& Basic heartbeats and timestamps. Expressive observers that are implemented using finite state machines, timed automata and hybrid automata. 
		& High
		& Yes
		& No
		\\\hline

	\end{tabular}

\end{table*}

==> tables/tab_resilientArchs.tex <==

\begin{table*}[tbhp]
	\centering
	\caption{Comparison of existing resilient architectures}

\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	
	& \multirow{ 2}{*}{\textbf{Architecture} }
	& \multicolumn{4}{c|}{\textbf{Features}} 
	& \multirow{ 2}{*}{\textbf{Target} } \\ 
	\cline{3-6}
	&
	&  \textbf{data collection}
	&  \textbf{fault detection}
	&  \textbf{fault containment}
	&  \textbf{adapt/reconfigure}
	&
	\\ 
	\cline{1-7}
	\multirow{5}{*}{\rotatebox[]{90}{\textbf{Self-Adaptive}} }
	&
	&  using probes and gauges
	&  Complex event processing~\cite{Luckham1998} 
	&  
	&  using effectors
	&  
	\\ 
	\cline{2-7}
	&&  &  &  &  &  \\ 
	
	\cline{2-7}
	&&  &  &  &  &  \\ 
	
	\cline{2-7} 
	&&  &  &  &  &  \\ 
	
	\cline{2-7} 
	&&  &  &  &  &  \\ 
	\hline 
\end{tabular} 
\end{table*}

==> tables/xlayerAnD.tex <==
\begin{tabular}{M{1.6cm}|M{2.2cm}|M{3cm}|@{}M{0pt}@{}} 
& \textbf{Resources} & \textbf{Requirements} &\\ \hline

\textbf{Application layer}
& NA
& End-to-end timing \tikzmark{a}~constraints, {S}ampling frequency, etc.,
&\\ [2ex]\hline 
\textbf{Platform layer}   
&  OS scheduler\tikzmark{b}, Network controller, Publisher-Subscriber, Fault tolerance, etc.                 
& Execution time, \tikzmark{d}Bandwidth,  
&\\ [2ex]\hline
\textbf{Physical layer}   
& Processor speed\tikzmark{c}, memory size and access latency, sensors/actuator response and recovery time, etc.           
& NA 
&\\ [2ex]\hline\\
\end{tabular}
\begin{tikzpicture}[overlay, remember picture, yshift=.25\baselineskip, shorten >=.5pt, shorten <=.5pt]
\draw [->, thick] ({pic cs:b}) [bend left] to ({pic cs:a});
\node[rotate=40, color=red] at (-3.8, 1.9)   (a) {availability};

\draw [->, thick] ([yshift=-5.75pt]{pic cs:a}) [bend left] to ([yshift=-5.75pt]{pic cs:b});
\node[rotate=40, color=red] at (-3.5, 1)   (a) {demand};

\draw [->, thick] ({pic cs:c}) [bend left] to ({pic cs:d});
\node[rotate=40, color=red] at (-3.4, 0.2)   (a) {availability};

\draw [->, thick] ([yshift=-5.75pt]{pic cs:d}) [bend left] to ([yshift=-5.75pt]{pic cs:c}); 
\node[rotate=40, color=red] at (-3.0, -0.8)   (a) {demand};
\end{tikzpicture}

%\tikzmark{a}{AAA} & \tikzmark{1}{111}
%\link{a}{b}
%\link{a}{2} 
